Active Learning for Network Traffic Classification: A Technical Study

Network Traffic Classification (NTC) has become an important feature in various network management operations, e.g., Quality of Service (QoS) provisioning and security services. Machine Learning (ML) algorithms as a popular approach for NTC can promise reasonable accuracy in classification and deal with encrypted traffic. However, ML-based NTC techniques suffer from the shortage of labeled traffic data which is the case in many real-world applications. This study investigates the applicability of an active form of ML, called Active Learning (AL), in NTC. AL reduces the need for a large number of labeled examples by actively choosing the instances that should be labeled. The study first provides an overview of NTC and its fundamental challenges along with surveying the literature on ML-based NTC methods. Then, it introduces the concepts of AL, discusses it in the context of NTC, and review the literature in this field. Further, challenges and open issues in AL-based classification of network traffic are discussed. Moreover, as a technical survey, some experiments are conducted to show the broad applicability of AL in NTC. The simulation results show that AL can achieve high accuracy with a small amount of data.

==> Table_1.tex <==
\begin{table*}[]
\centering
\caption{Summary of papers on Active Learning Challenges \textcolor{red}{This table should have larger text}}
\label{table_example1}
\tiny
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Challenge} & \textbf{Noisy annotation}  &\textbf{Stopping criteria}  &\textbf{Outliers in the data } & \textbf{Drifting distribution} & \textbf{Instance selection criteria} \\ \hline
\textbf{Source}    &  \cite{donmez2008proactive}, \cite{nguyen2004active}, \cite{donmez2007dual}  & \cite{hakkani2006active}, \cite{altschuler2019stopping}, \cite{bloodgood2014method}, \cite{temerinac2015deciding}& \cite{yang2009outlier}, \cite{ramaswamy2000efficient}, \cite{breunig2000lof}, \cite{warner2008applied} & \cite{hakkani2006active}, \cite{yang2011active}, \cite{vzliobaite2013active} & \cite{wang2015active}, \cite{freytag2014selecting}, \cite{bouguelia2016adaptive} \\ \hline



\end{tabular}
\end{table*}

==> sections/challenges.tex <==
\section{Challenges of using \gls{al} in \gls{ntc}}
\label{sec:challenges}
Although \gls{al} can achieve a reasonable level of accuracy using much less labeled examples than traditional ML algorithms, there are still some unsolved problems listed below: %In this section, the key issues and challenges of \gls{al} are discussed. 
\begin{itemize}
\item \textbf{Noisy annotation:} In conventional ML, the labels are often assumed to be the ground truth without noise; However, when the instances are annotated by humans or machines that are prone to errors, additional considerations must be made \cite{artstein2008inter}. \textcolor{black}{The existence of noisy labels is problematic for the uncertainty sampling strategy, due to the fact that this strategy is intrinsically noise-seeking \cite{GARCIA2015108}. In networking, noises can be generated deliberately or accidentally. Intruders can generate packets to mislead NTC systems. For example, in \cite{perdisci2006misleading} the problem of noise in the worm signatures extraction algorithms has been investigated. In these algorithms, deliberate noise can prevent from building reliable and useful worm signatures, and consequently decline the performance of IDSs. Noises can also be generated accidentally based on human or automated process labeling mistakes. In \cite{donmez2008proactive}, Donmez et al. proposed proactive learning to deal with noisy labels as it uses a decision-theoretic method in order to jointly choose the optimal oracle and instance. %In \cite{nguyen2004active}, the authors incorporate clustering into \gls{al} to improve the performance of classification. The introduced approach allows to choose the most informative instances. In another study carried out by Donmez et al. \cite{donmez2007dual}, a dynamic approach, namely dual \gls{al} was proposed. In this approach, to avoid falling into local maximum, the authors combined density-weighted uncertainty sampling and standard uncertainty sampling.}
}
\item \textbf{Stopping criteria:} The stopping criteria determine when to stop querying unlabeled instances. Several criteria for determining a good stopping point have been proposed, such as reaching the desired accuracy, running time, or limiting the number of queries.
% However, determining the best stopping criteria remains highly controversial. 
In terms of applying \gls{al} on \gls{ntc}, the stopping criteria should also satisfy the challenges of using \gls{ml} techniques in \gls{ntc}, mainly to improve the time complexity of the \gls{al} technique to re-train the model. As an example, achieving the desired accuracy may cause consuming an unreasonable time resulting in an unused training model.
\textcolor{black}{Many studies on \gls{al} considered the convergence of the error rate on a set of unseen data as the stopping criterion. Nevertheless, providing a new annotated unseen dataset is in direct contradiction to the goal of \gls{al}, due to the fact that the purpose is to reduce the need for annotation. In addition, if the unseen dataset contains a small number of instances, there are no guarantees that this dataset will be representative of the future instances. To alleviate this challenge, the authors in \cite{hakkani2006active} proposed a novel active approach, in which the active model itself chooses the most informative instances for its training, uses active evaluation to evaluates itself, and re-trains itself when necessary.}

%In other words, they use the convergence of error rate on the training set as a stopping criterion to decide on-demand labeling. 
%In another work by Altschuler and Bloodgood \cite{altschuler2019stopping}, a new stopping method, called Predicted Change of F Measure, has been introduced to reduce annotation cost without affecting performance. Indeed, this work is an improved version of the work conducted by Bloodgood and Vijay-Shanker \cite{bloodgood2014method}, in which \gls{al} ends when the forecasting at different iterations stabilizes. Temerinac-Ott et al. \cite{temerinac2015deciding} proposed efficient stopping criteria for \gls{al} in the drug-target prediction. In their work, they adopted batch-wise learning, in which a fixed number of instances is sampled in each learning round. Each learning round determines a time point in the \gls{al} system and is calculated according to the number of batches of instances sampled. For each time point, the performance of the model is forecasted. The \gls{al} process is ended, for example, if a certain cost of instance sampling is reached or the forecasted performance of the model is reasonable.  }

\input{Table 1}

\item \textbf{Outliers in the data:} In a canonical definition, an outlier is a data example that considerably differs from other data points in a dataset, and may occur by chance or be due to an experimental error resulting in inefficiency to analyze the overall behavior of the dataset. Labeling outlier instances by a human/machine annotator may not help in the prediction of the labels of unlabeled instances, because these instances are likely to be representative of a small number of instances. %\textcolor{black}{The existence of outliers data can increase variance in your dataset, which declines statistical power. Thus, keeping outliers out can lead to more meaningful results in terms of statistically.
 %As an example, in network time-series dataset, if the data points show the delay of packets, outliers can appear because of jitter in data forwarding called global outliers. Network congestion can also cause collective outliers as the trend of the time-series changed for a short period of time. }

\textcolor{black}{{In \gls{ntc} data, outliers appears based on networking challenges, \eg inefficient data forwarding models and network congestion.} There are two major approaches to deal with outliers, including correcting and removing outlier data. To remove outliers, one can use a set of methods, however, methods such as Z-Score, smoothing techniques, and interquartile range (IQR)-Score are more common.} %Note that removing outliers is the right choice only in specific situations. It is crucially important to understand how outliers are introduced to the dataset, e.g. by mistake during the collecting process or they are showing the variance in your dataset, and it is possible to occur again.  This is mainly due to the fact that outliers can be quite knowledgeable about the subject-field.} 
Correction of outliers is another key approach to deal with outlier data. Apart from the dealing method, The first step towards handling outliers is outliers detection. There are tons of methods for outliers detection. The model-based method is among the simplest outliers detection methods, in which one constructs a model for all instances, and then defines outliers as instances having significant deviations from the constructed profiles \cite{yang2009outlier}. The proximity-based method is another extensively adopted method for outliers detection. %The main idea behind this method is to answer this question that to what extent the point is rare. 
This can be done through algorithms such as K-th nearest neighbor and the ratio of local reachability density \cite{ramaswamy2000efficient}, \cite{breunig2000lof}. \textcolor{red}{Generally speaking,  both correcting and removing outlier solutions can be applied to \gls{ntc} techniques. Practically, outlier correction techniques are more complicated to apply, as they need to detect outliers and correct them which is a time- and resource-consuming task. The main advantage of outlier correction techniques is that they can be useful in case of data scarcity as more data can generally help \gls{ml} techniques to be trained efficiently. In case of speed, outlier remover solutions are more efficient.  The characteristic of real-world applications, \eg available resource and delay-sensitive can help to make a decision on which approach is more efficient. } 

%After taking outliers detection step, one may need to use outliers correction methods to lower the impact of outlier data. Log transformation is one of the widely used methods to deal with the variability of data. This method can shift outlier instances at the high end of a distribution closer to the mean in order to make the distribution as normal as possible. Using this method, it is expected that it lends a certain validity to the related statistical analyses \cite{warner2008applied}. %The nonparametric statistical ranking is another popular technique to reduce the impact of outliers through the transformation of measures to ranks\cite{zimmerman1990relative}. In addition, Winsorizing can be used as a method to correct outlier data \cite{dixon1974trimming}. Winsorization refers to replacing an outlier data point (extreme value) with a smaller data value. One can use different percentile of data-dependent values for this replacement. 

\item \textbf{Drifting distribution:} Most existing \gls{al} algorithms work on the assumption that the data is \gls{iid}; However, the selection of instances based on a non-random distribution, which shifts over time, may lead to divergence between the prior distribution of instances and the current one. Such divergence can affect the performance of the learning task (i.e. classification or regression), since \gls{iid} assumption is no longer valid. \textcolor{black}{In \gls{ntc}, drifting distribution in gathered data from the network that can appear because of different events, \eg network congestion, inefficient queuing models in middle nodes while data is transferring from source to destination, and inefficient packet inspection model.}
%\textcolor{black}{The work presented in \cite{yang2011active}, explored \gls{al} under distribution drift. The author considers a stream-based selective sampling and allows the distribution of the instances to shift over time. In this work, comprehensive analyses were performed to investigate the problem of distribution drift in \gls{al}. Moreover, the author proposed a framework to solve the problem. The work in \cite{hakkani2006active} proposed to combine the Kullback–Leibler divergence between the distribution from the prior model and from the constructed model in order to solve the problem. Žliobaite et al. \cite{vzliobaite2013active} focused on \gls{al} in the presence of streaming data. They explain that an \gls{al} task can be compounded by the fact that the streaming data distribution may change over time. Towards isolating the impact of the distribution drift,  a framework for \gls{al} from streaming data with drifting distributions is established. Furthermore,  three \gls{al} strategies are proposed that are able to handle drift streaming data.}
\item \textbf{Instance selection criteria:} As previously mentioned, a query strategy deals with selecting the instances that would be more useful to improve the accuracy of the learning model if labeled. Hence, criteria are established to select the instances that are important for an \gls{al} system, as the system uses the selected instances like a training set. Several query strategies have been proposed in the previous \gls{al} literature \cite{dasgupta2005analysis, dirkse2019active}; however, there is a lack of research on the role of the annotator (human or machine) in the labeling process. In other words, the annotator plays a passive role in providing a label to an instance, and a lack of understanding about the importance of querying is apparent. \textcolor{black}{In \gls{ntc}, labeling is an important process especially for new-unknown network traffics that are started without any notification, \eg a multimedia stream started by a smartphone. In addition, different query strategies can be employed based on the volume of existing samples and the essence of the network traffic. Based on the \textit{theory of network} challenge, there is no specific policy to use query strategies as the behaviors of the networks are different.}. %\textcolor{black}{In \cite{wang2015active}, Wang et al. proposed a novel querying framework, in which two key \gls{al} scenarios, query synthesis and pool-based sampling, are combined. In the proposed framework, to select an instance to label, first it uses the labeled instances to synthesize an instance in the neighborhood of the decision boundary. Then, it chooses the real instance that is close enough to the synthesized instance as a query. Freytag et al. \cite{freytag2014selecting} have reported that they have developed an effective query strategy that outperforms state-of-the-art on multiple datasets. The proposed strategy is based on measuring the anticipating change in the outputs of the model when an unlabeled instance would be labeled and included in the training process. The work of Bouguelia et al. \cite{bouguelia2016adaptive} introduced a new query strategy, namely sufficient weight, where they used instance weighting to enhance the performance of the \gls{al} system. Specifically, the proposed strategy first determines the smallest weight needed to change the learner's prediction about the class label of instance. If the selected weight is small enough to change the label prediction, the learner is uncertain about the new instance and the true label of the instance is needed to be queried.}
\item \textbf{Labeling method:} \textcolor{red}{Although Section \ref{sec:performance} shows that \gls{al} techniques are efficient in case of \gls{ntc}, especially improving the training time and dealing with the shortage of data samples, the main drawback of using \gls{al} is the lack of a concrete labelling technique. Due to the \gls{Concept Drift} challenge, the model should be retrained frequently. On the other hand, as mentioned above, labelling the selected instances can be performed by human or machine,  but in real-world applications of \gls{ntc}, using the human-labour is almost impossible, due to the speed and inefficiency problems. Considering that in most real-world applications of networking, data are unlabeled or semi-labeled \cite{alsheikh2016mobile}, a machine-based labeling method is highly needed that can be adapted by the speed of the network with a high accuracy in labeling to be applied \gls{al} in real-world applications of \gls{ntc}.}
\end{itemize}

The works that consider solving the challenge are summarized in Table \ref{table_example1}. We observe that different techniques have been used to solve different issues in different \gls{al} systems. Regarding traffic classification tasks, it can be argued that the most crucial issue is drifting distribution. This is mainly due to the fact that many traffic classification applications such as \gls{ids} have to update their database by injecting new instances or using stream-based sampling.


==> sections/futuredirections.tex <==
\section{Future Direction and Open Issues}
\label{sec:future}
In this section, we discuss future directions and open issues based on our findings in terms of using \gls{al} in \gls{ntc}.
\begin{enumerate}
 \item \textbf{Lack of close collaboration between deep learning and \gls{al} techniques:} As we mentioned, the lack of labeled data is a serious problem in using \gls{ml} techniques in many real-world applications, especially networking. Meanwhile, deep learning models are already being deployed in a diverse range of real-world applications, such as self-driving cars, anomaly detection, wearables, \gls{ntma} \cite{abbasi2021deep} and healthcare. However, to reach the full potential of deep learning in such applications, the lack of labeled data is one of the major barriers. Most recent works in the context of \gls{al} focus on proposing new/improved algorithms, and few of them deal with the problem of intelligent data collection \cite{2020arXiv200900236R}. From a data science perspective, it is desirable to fill this gap. We believe that conducting further research on deep \gls{al} \cite{pimentel2018deep} and human-in-the-loop \gls{ml} \cite{yang2018active} will narrow the gap. In these branches of \gls{ml}, intelligent data collection is a step of the \gls{ml} process. Human-in-the-loop \gls{ml} can further facilitate the process of labeling difficult/new instances that a machine annotator cannot handle. 
 
 \item \textbf{NTMA applications in which \gls{al} is still missing:} 
 As mentioned above, many \gls{al} works deploy \gls{al} for security purposes, such as intrusion detection and malware detection. However, there is still a long list of \gls{al} applications, such as traffic forecasting,fault management, \gls{qos} provisioning, and routing, in which AL has not been employed. For instance, to our best knowledge, no studies have been conducted on the coupling of network traffic prediction with AL. This is maybe due to the dynamic nature of traffic prediction tasks and difficulty of working with streaming data. The traffic load on communication networks changes overtime or in different situations. Indeed, the distribution of the traffic load may face the problem of drift distribution.
 
 \item \textbf{Lack of appropriate and public network traffic datasets:} \gls{ntc} involves the categorization of network traffic into several traffic classes, such as WWW, mail, attack, P2P, and multimedia. However, as mentioned above, network security becomes a dominant application of \gls{al}-based traffic classification. For example, we have found only two papers that have used \gls{al} for \gls{p2p} traffic classification \cite{dai2012peer}, \cite{liu2015active}. This is because there are few relevant and public non-security related traffic datasets. Moreover, the existing datasets that are widely used in these papers are often not updated. The ever-growing popularity in using encryption protocols and the number of Internet-based applications, calls for up-to-date non-security related traffic datasets to employ for \gls{ml} techniques. \textcolor{black}{ Although Theory of Network challenge shows benchmark datasets are unable to train the ML models to be used in all networks, having the datasets can help to evaluate the performance of \gls{ml} techniques \eg \gls{al} in \gls{ntc}.}
 
 \item \textbf{Uncertainty in the performance of \gls{al} based on \textit{Theory of Network}:} Although the performance of \gls{al} is evaluated based on benchmark datasets, there is no guarantee to have such performance in each network separately. Different reasons \eg weak samples, \gls{ml} techniques, the complexity of network traffics, etc. can affect the performance of the \gls{al} in each network. Over-fitting can be a considerable challenge in different networks regarding the use of \gls{al}. Although in this study, we evaluate the performance of \gls{al} in a general manner, its performance should be considered in real-world networks. 
 
 \item \textbf{Resource-constraint networks:} Most \gls{ml} techniques including \gls{al} are designed to be performed by resource-rich devices, but in real-world applications, there is a considerable need to optimize \gls{ml} techniques to be performed by weak devices. As different computing paradigms are emerging \eg Fog and Edge, network managers tend to employ weak devices to perform resource-consuming tasks \ie \gls{ml} techniques. Different distributed learning techniques are introduced to use resources in weak devices to perform \gls{ml} techniques \eg federated learning \cite{yang2019federated}, that can be mixed with \gls{al} techniques.
 
 \item \textbf{Labeling time:} As the training time of the \gls{al} techniques are considerably low because of a few samples, labeling can be potentially time consuming that causes a challenge for time-sensitive \gls{ntc} applications. Due to the properties of \gls{ntc}, labeling techniques should be optimized in terms of time-complexity.
 
 \item \textbf{Mixing Stopping Criteria to satisfy \gls{ntc} requirements:} As \gls{ntc} is sensitive in both time and accuracy aspects, providing efficient stopping criteria that can satisfy its requirements is necessary. The criteria are application-based meaning that it should be selected based on each network traffic separately. As an example, in case of providing security for network traffic, accuracy has a higher priority, but multimedia streams are mainly time-sensitive.  
 \end{enumerate}
